Unlocking Blocked Communicating Processes

We study the problem of disentangling locked processes via code refactoring. We identify and characterise a class of processes that is not lock-free; then we formalise an algorithm that statically detects potential locks and propose refactoring procedures that disentangle detected locks. Our development is cast within a simple setting of a finite linear CCS variant \^a although it suffices to illustrate the main concepts, we also discuss how our work extends to other language extensions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{23}
\providecommand{\publicationstatus}{M.H. ter Beek and A. Lluch Lafuente (Eds.): 11th International Workshop\\
on Automated Specification and Verification of Web Systems (WWV'15).\\
EPTCS 188, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.188.4}{10.4204/EPTCS.188.4}}

